BAFFLE : Blockchain Based Aggregator Free Federated Learning

A key aspect of Federated Learning (FL) is the requirement of a centralized aggregator to maintain and update the global model. However, in many cases orchestrating a centralized aggregator might be infeasible due to numerous operational constraints. In this paper, we introduce BAFFLE, an aggregator free, blockchain driven, FL environment that is inherently decentralized. BAFFLE leverages Smart Contracts (SC) to coordinate the round delineation, model aggregation and update tasks in FL. BAFFLE boosts computational performance by decomposing the global parameter space into distinct chunks followed by a score and bid strategy. In order to characterize the performance of BAFFLE, we conduct experiments on a private Ethereum network and use the centralized and aggregator driven methods as our benchmark. We show that BAFFLE significantly reduces the gas costs for FL on the blockchain as compared to a direct adaptation of the aggregator based method. Our results also show that BAFFLE achieves high scalability and computational efficiency while delivering similar accuracy as the benchmark methods.

==> DecentAI_blockchain2020_camera_ready/junk.tex <==

%However, there is a lack of a scalable, blockchain based decentralized FL framework that incurs low computational costs, but yet retains the benefits of an aggregator free setting \cite{harris2019decentralized}.
%Therefore, the need of the hour is a scalable, blockchain based decentralized FL scheme that incurs low computational costs, but yet retains the benefits of an aggregator free setting \cite{harris2019decentralized}. 

%Lastly, an aggregator free FL technique would significantly empower small organizations to collaboratively develop a global AI model without requiring excessive skills and expertise in deploying cloud applications.

%Lastly, small organizations, not having the skill and expertise in the cloud computing domain, could use a blockchain based FL approach to learn from each others experiences to collaboratively develop a global AI model without sharing private data. 

%However, a key challenge in a blockchain driven aggregator free FL scheme would inevitably incur prohibitive costs its high cost and computational scalability \cite{harris2019decentralized}. 

%A blockchain based FL scheme, eliminates the aggregator through the use of SmartContracts(SC).    

%Although blockchain based FL mechanisms have been proposed \cite{weng2019deepchain,lyu2019towards} in the past, 
% the computational constraints that need to be considered in order to make the FL process aggregator free have so far not been considered.  

% Even though blockchain driven incentive mechanisms have been proposed for enabling trust and fairness \cite{weng2019deepchain,lyu2019towards} in FL applications, . 

%in order to alleviate the 
%which can greatly alleviate the operational concerns with a centralized aggregator mechanism.

%investigate the use of blockchain as a means to eliminate the computational and operational limitations induced by a cloud based aggregator.

%In this paper, we investigate the use of blockchain as a means to eliminate the computational and operational limitations induced by a cloud based aggregator.


% Therefore, as a result of the central aggregator, high barriers of entry are introduced which render the benefits of FL inaccessible to micro enterprises and social organizations which might lack the scale and sophistication to launch and manage their own large scale FL tasks. 

% trust their aggregator's ability to carry out the selection and aggregation of local models.

% Despite its privacy benefits, the centralized nature of the aggregator faces numerous operational challenges. First, the selection and updation steps carried out by the aggregator must be fair to all users. Second, all users  

% Despite its privacy benefits, the centralized nature of the aggregator faces numerous operational challenges. First, in FL applications, end users are assumed to trust their aggregator's ability to carry out the selection and aggregation of local models. However, such an assumption could be highly misplaced since an aggregator can potentially exhibit bias towards a select few user devices \cite{}. Second, the scope of FL is restricted to applications where a centralized aggregator is feasible \cite{he2019central}. 

% As a result, an aggregator's resiliency depends on the robustness of the cloud infrastructure. Owing to a rather centralized nature of cloud based systems, a failure at the cloud level could significantly influence performance of the FL framework. Lastly, the same cloud based computational framework needs to be individually instantiated for every FL task which in turn leads to separate instantiations of the centralized aggregator as well. 
% Therefore, a scalable, cloud based FL framework for a single learning task demands a high barrier for participation in terms of resources and expertise. Such restrictions render the benefits of FL inaccessible to micro enterprises and social organizations which might lack the scale and sophistication to launch and manage their own large scale FL tasks.


% However, the centralized nature of the aggregator leads to trust and resiliency concerns \cite{roy2019braintorrent}. Moreover, it might be infeasible to set up a central server due to operational reasons \cite{he2019central}.  

%numerous computational and operational challenges are induced in the FL process.


%whats wrong with a centralized aggregator
% Specifically, the centralized nature of the aggregator in a FL environment, leads to concerns about trustworthiness, fairness and resiliency. First, in FL applications, an aggregator can potentially exhibit bias towards a select few user devices \cite{lyu2019towards}. Second, the centralized aggregator is usually cloud based \cite{fl2} introduces the ques.
% end users are assumed to trust their aggregator to carry out the selection and aggregation of local models in a fair and impartial manner \cite{FL_Original}. However, such an assumption could be highly misplaced since .  As a result, an aggregator's resiliency depends on the robustness of the cloud infrastructure. Owing to a rather centralized nature of cloud based systems, a failure at the cloud level could impact the FL mechanism as well. Moreover, access to a cloud environment, necessary for a centralized aggregator, might be out of reach for small and micro scale enterprises due to lack of technical skill and expertise \cite{carcary2014adoption}. Therefore, such high barriers of entry render the benefits of FL inaccessible to micro enterprises and social organizations which might lack the scale and sophistication to launch and manage their own large scale FL tasks. 


%However, due to the centralized nature of the aggregator, numerous computational and operational challenges are induced in the FL process 

%In reality

%Despite privacy benefits of FL, the presence of a central aggregator often leads to questions about its trustworthiness \cite{weng2019deepchain}, fairness \cite{lyu2019towards} and resiliency \cite{kim2018device}. 

%Computationally, the entire FL process is divided into rounds . In each round, an aggregator selects a set of user devices and integrates copies of their locally trained machine learning model into a globally held model. 

%Computationally, the FL paradigm functions in an iterative fashion wherein every iterative step is referred to as a round. In the beginning of every round, a copy of a globally available machine learning model is pushed to select end user devices. Each selected device trains the global copy on the local data set to determine a new local estimate of the global model. Local estimates from all selected devices are averaged to yield the next estimate of the global model which signals the culmination of the round. 

%challenges with federated learning in the current context: role of the aggregator

% %whats wrong with a centralized aggregator
% Specifically, the centralized nature of the aggregator in a FL environment, leads to questions about trustworthiness, fairness and resiliency \cite{lyu2019towards,kim2018device}. First, in FL applications, end users are assumed to trust their aggregator to be honest and carry out the selection and aggregation of local models in a fair and impartial manner \cite{lyu2019towards}. However, such an assumption could be highly misplaced since an aggregator can potentially exhibit bias towards a select few user devices \cite{lyu2019towards}. Second, the scope of FL is restricted to applications where a centralized aggregator is orchestrated on the cloud \cite{fl2,lyu2019towards,kim2018device}. As a result, an aggregator's resiliency depends on the robustness of the cloud infrastructure. Owing to a rather centralized nature of cloud based systems, a failure at the cloud level could impact the FL mechanism as well \cite{kim2018device}. Moreover, access to a cloud environment, necessary for a centralized aggregator, might be out of reach for small and micro scale enterprises due to lack of technical skill and expertise \cite{carcary2014adoption}. Therefore, such high barriers of entry render the benefits of FL inaccessible to micro enterprises and social organizations which might lack the scale and sophistication to launch and manage their own large scale FL tasks. 

%Blockchain presents a viable alternative to address the issues of trust 

% the inability to set up a scalable, resilient cloud based aggregator 
% such restrictions render the benefits of FL inaccessible to micro enterprises and social organizations which might lack the scale and sophistication to launch and manage their own large scale FL tasks. 

% Moreover, 
% demands a high barrier of entry in terms of technical expertise and manpower \cite{carcary2014adoption}.  as their larger counterparts,  investment costs \cite{cld2}. Therefore, 
% %Lastly, 
% %lack of cloud readiness proves to be a significant hurdle in adoption  
% %on account of a high barrier of entry 
% %achieving scalability in a cloud environment requires a high barrier of entry %on account of 

% Lastly, a scalable, cloud based FL framework for a single learning task demands a high barrier for participation in terms of resources and expertise. Moreover, such restrictions render the benefits of FL inaccessible to micro enterprises and social organizations which might lack the scale and sophistication to launch and manage their own large scale FL tasks. 

%how does blockchain help?
% The use of blockchain has been shown to address issues of trust \cite{weng2019deepchain}, fairness \cite{lyu2019towards} and resiliency \cite{kim2018device} in the field of federated and distributed learning.  
% %The use of blockchains have been proposed within the fields of federated and distributed learning to implement incentive mechanisms \cite{kim2018device}, prove auditability of data \cite{weng2019deepchain} and ensure fairness among participants \cite{lyu2019towards}. 
% However a blockchain based decentralized learning mechanism that preserves data privacy of users by only aggregating model updates on the chain remains an open challenge \cite{harris2019decentralized}.  

%given the significant costs associated with the model aggregation process, a blockchain based mechanism is sought that is computationally efficient, 
%Therefore, preserving data privacy of participants by only aggregating model updates on a blockchain based ML platform seems to be 
%In this paper, we investigate the use of blockchain for orchestrating 
%preserving data privacy of participants by only aggregating model updates on a blockchain based ML platform seems to be 



==> junk.tex <==

%However, there is a lack of a scalable, blockchain based decentralized FL framework that incurs low computational costs, but yet retains the benefits of an aggregator free setting \cite{harris2019decentralized}.
%Therefore, the need of the hour is a scalable, blockchain based decentralized FL scheme that incurs low computational costs, but yet retains the benefits of an aggregator free setting \cite{harris2019decentralized}. 

%Lastly, an aggregator free FL technique would significantly empower small organizations to collaboratively develop a global AI model without requiring excessive skills and expertise in deploying cloud applications.

%Lastly, small organizations, not having the skill and expertise in the cloud computing domain, could use a blockchain based FL approach to learn from each others experiences to collaboratively develop a global AI model without sharing private data. 

%However, a key challenge in a blockchain driven aggregator free FL scheme would inevitably incur prohibitive costs its high cost and computational scalability \cite{harris2019decentralized}. 

%A blockchain based FL scheme, eliminates the aggregator through the use of SmartContracts(SC).    

%Although blockchain based FL mechanisms have been proposed \cite{weng2019deepchain,lyu2019towards} in the past, 
% the computational constraints that need to be considered in order to make the FL process aggregator free have so far not been considered.  

% Even though blockchain driven incentive mechanisms have been proposed for enabling trust and fairness \cite{weng2019deepchain,lyu2019towards} in FL applications, . 

%in order to alleviate the 
%which can greatly alleviate the operational concerns with a centralized aggregator mechanism.

%investigate the use of blockchain as a means to eliminate the computational and operational limitations induced by a cloud based aggregator.

%In this paper, we investigate the use of blockchain as a means to eliminate the computational and operational limitations induced by a cloud based aggregator.


% Therefore, as a result of the central aggregator, high barriers of entry are introduced which render the benefits of FL inaccessible to micro enterprises and social organizations which might lack the scale and sophistication to launch and manage their own large scale FL tasks. 

% trust their aggregator's ability to carry out the selection and aggregation of local models.

% Despite its privacy benefits, the centralized nature of the aggregator faces numerous operational challenges. First, the selection and updation steps carried out by the aggregator must be fair to all users. Second, all users  

% Despite its privacy benefits, the centralized nature of the aggregator faces numerous operational challenges. First, in FL applications, end users are assumed to trust their aggregator's ability to carry out the selection and aggregation of local models. However, such an assumption could be highly misplaced since an aggregator can potentially exhibit bias towards a select few user devices \cite{}. Second, the scope of FL is restricted to applications where a centralized aggregator is feasible \cite{he2019central}. 

% As a result, an aggregator's resiliency depends on the robustness of the cloud infrastructure. Owing to a rather centralized nature of cloud based systems, a failure at the cloud level could significantly influence performance of the FL framework. Lastly, the same cloud based computational framework needs to be individually instantiated for every FL task which in turn leads to separate instantiations of the centralized aggregator as well. 
% Therefore, a scalable, cloud based FL framework for a single learning task demands a high barrier for participation in terms of resources and expertise. Such restrictions render the benefits of FL inaccessible to micro enterprises and social organizations which might lack the scale and sophistication to launch and manage their own large scale FL tasks.


% However, the centralized nature of the aggregator leads to trust and resiliency concerns \cite{roy2019braintorrent}. Moreover, it might be infeasible to set up a central server due to operational reasons \cite{he2019central}.  

%numerous computational and operational challenges are induced in the FL process.


%whats wrong with a centralized aggregator
% Specifically, the centralized nature of the aggregator in a FL environment, leads to concerns about trustworthiness, fairness and resiliency. First, in FL applications, an aggregator can potentially exhibit bias towards a select few user devices \cite{lyu2019towards}. Second, the centralized aggregator is usually cloud based \cite{fl2} introduces the ques.
% end users are assumed to trust their aggregator to carry out the selection and aggregation of local models in a fair and impartial manner \cite{FL_Original}. However, such an assumption could be highly misplaced since .  As a result, an aggregator's resiliency depends on the robustness of the cloud infrastructure. Owing to a rather centralized nature of cloud based systems, a failure at the cloud level could impact the FL mechanism as well. Moreover, access to a cloud environment, necessary for a centralized aggregator, might be out of reach for small and micro scale enterprises due to lack of technical skill and expertise \cite{carcary2014adoption}. Therefore, such high barriers of entry render the benefits of FL inaccessible to micro enterprises and social organizations which might lack the scale and sophistication to launch and manage their own large scale FL tasks. 


%However, due to the centralized nature of the aggregator, numerous computational and operational challenges are induced in the FL process 

%In reality

%Despite privacy benefits of FL, the presence of a central aggregator often leads to questions about its trustworthiness \cite{weng2019deepchain}, fairness \cite{lyu2019towards} and resiliency \cite{kim2018device}. 

%Computationally, the entire FL process is divided into rounds . In each round, an aggregator selects a set of user devices and integrates copies of their locally trained machine learning model into a globally held model. 

%Computationally, the FL paradigm functions in an iterative fashion wherein every iterative step is referred to as a round. In the beginning of every round, a copy of a globally available machine learning model is pushed to select end user devices. Each selected device trains the global copy on the local data set to determine a new local estimate of the global model. Local estimates from all selected devices are averaged to yield the next estimate of the global model which signals the culmination of the round. 

%challenges with federated learning in the current context: role of the aggregator

% %whats wrong with a centralized aggregator
% Specifically, the centralized nature of the aggregator in a FL environment, leads to questions about trustworthiness, fairness and resiliency \cite{lyu2019towards,kim2018device}. First, in FL applications, end users are assumed to trust their aggregator to be honest and carry out the selection and aggregation of local models in a fair and impartial manner \cite{lyu2019towards}. However, such an assumption could be highly misplaced since an aggregator can potentially exhibit bias towards a select few user devices \cite{lyu2019towards}. Second, the scope of FL is restricted to applications where a centralized aggregator is orchestrated on the cloud \cite{fl2,lyu2019towards,kim2018device}. As a result, an aggregator's resiliency depends on the robustness of the cloud infrastructure. Owing to a rather centralized nature of cloud based systems, a failure at the cloud level could impact the FL mechanism as well \cite{kim2018device}. Moreover, access to a cloud environment, necessary for a centralized aggregator, might be out of reach for small and micro scale enterprises due to lack of technical skill and expertise \cite{carcary2014adoption}. Therefore, such high barriers of entry render the benefits of FL inaccessible to micro enterprises and social organizations which might lack the scale and sophistication to launch and manage their own large scale FL tasks. 

%Blockchain presents a viable alternative to address the issues of trust 

% the inability to set up a scalable, resilient cloud based aggregator 
% such restrictions render the benefits of FL inaccessible to micro enterprises and social organizations which might lack the scale and sophistication to launch and manage their own large scale FL tasks. 

% Moreover, 
% demands a high barrier of entry in terms of technical expertise and manpower \cite{carcary2014adoption}.  as their larger counterparts,  investment costs \cite{cld2}. Therefore, 
% %Lastly, 
% %lack of cloud readiness proves to be a significant hurdle in adoption  
% %on account of a high barrier of entry 
% %achieving scalability in a cloud environment requires a high barrier of entry %on account of 

% Lastly, a scalable, cloud based FL framework for a single learning task demands a high barrier for participation in terms of resources and expertise. Moreover, such restrictions render the benefits of FL inaccessible to micro enterprises and social organizations which might lack the scale and sophistication to launch and manage their own large scale FL tasks. 

%how does blockchain help?
% The use of blockchain has been shown to address issues of trust \cite{weng2019deepchain}, fairness \cite{lyu2019towards} and resiliency \cite{kim2018device} in the field of federated and distributed learning.  
% %The use of blockchains have been proposed within the fields of federated and distributed learning to implement incentive mechanisms \cite{kim2018device}, prove auditability of data \cite{weng2019deepchain} and ensure fairness among participants \cite{lyu2019towards}. 
% However a blockchain based decentralized learning mechanism that preserves data privacy of users by only aggregating model updates on the chain remains an open challenge \cite{harris2019decentralized}.  

%given the significant costs associated with the model aggregation process, a blockchain based mechanism is sought that is computationally efficient, 
%Therefore, preserving data privacy of participants by only aggregating model updates on a blockchain based ML platform seems to be 
%In this paper, we investigate the use of blockchain for orchestrating 
%preserving data privacy of participants by only aggregating model updates on a blockchain based ML platform seems to be 


